Securing Secure Aggregation: Mitigating Multi-Round Privacy Leakage in Federated Learning

Secure aggregation is a critical component in federated learning (FL), which enables the server to learn the aggregate model of the users without observing their local models. Conventionally, secure aggregation algorithms focus only on ensuring the privacy of individual users in a single training round. We contend that such designs can lead to significant privacy leakages over multiple training rounds, due to partial user selection/participation at each round of FL. In fact, we show that the conventional random user selection strategies in FL lead to leaking users' individual models within number of rounds that is linear in the number of users. To address this challenge, we introduce a secure aggregation framework, Multi-RoundSecAgg, with multi-round privacy guarantees. In particular, we introduce a new metric to quantify the privacy guarantees of FL over multiple training rounds, and develop a structured user selection strategy that guarantees the long-term privacy of each user (over any number of training rounds). Our framework also carefully accounts for the fairness and the average number of participating users at each round. Our experiments on MNIST and CIFAR-10 datasets in the IID and the non-IID settings demonstrate the performance improvement over the baselines, both in terms of privacy protection and test accuracy.

==> 08-Impossibility-Proof.tex <==

In this appendix, we study the optimal trade-off between the multi-round privacy guarantee and the average aggregation cardinality. Since the average aggregation cardinality depends on the number of distinct sets used in the selection strategy, we focus on establishing an upper bound on this number of distinct set given a multi-round privacy $T$.   

% Specifically, we  consider the following question. 
% \emph{Q: Given a multi-round privacy guarantee $T$,  what is the maximum number of distinct $K$-user sets that the server can choose from?}

We denote the maximum number of distinct sets by $R_{\mathrm{max}}$ and we derive an upper bound next.  The key idea of our bound is that every two distinct sets $\mathcal S^{(i)}$ and $\mathcal S^{(j)}$ cannot have in common more than $K-\floor*{T/2}$ users. That is, we must have 
\begin{align}
\label{eqn:necessary}
|\mathcal S^{(i)} \cap \mathcal S^{(j)}| \leq K-\floor*{T/2}.
\end{align}
Otherwise, the server can compute 
$\sum_{l \in \mathcal S^{(i)}} \mathbfsl x_l-\sum_{l \in \mathcal S^{(j)}} \mathbfsl x_l$, which leads to a privacy violation as 
\begin{align}
\| \sum_{l \in \mathcal S^{(i)}} \mathbfsl x_l-\sum_{l \in \mathcal S^{(j)}} \mathbfsl x_l \|_0 < T.
\end{align}
We provide our upper bound in Theorem \ref{thm:impossibility}.

\begin{theorem}
\label{thm:impossibility}
The maximum number of distinct sets of weight $K$ of any strategy guaranteeing a privacy $T$ is upper bounded as follows
\begin{align}
    R_{\mathrm{max}} \leq \frac{\binom{N}{K-\floor*{T/2}+1}}{\binom{K}{K-\floor*{T/2}+1}}.
\end{align}
% and when $N>N_0(k)$, we have 
% \begin{align}
%     R_{\mathrm{max}}  \leq \prod\limits_{i=0}^{K-\ceil*{T/2}} \frac{N-i}{K-i}=\frac{\binom{N}{K}}{\binom{N-K+\ceil*{T/2}-1}{\ceil*{T/2}-1}}.
% \end{align}
% We also have
% \begin{align}
%     R_{\mathrm{max}} \leq \frac{\binom{N}{K-\ceil*{T/2}+1}}{\binom{K}{K-\ceil*{T/2}+1}}.
% \end{align}
\end{theorem}
Before proving Theorem \ref{thm:impossibility}, we begin by recalling the following useful facts about \emph{$L$-systems} \cite{ray1975t,deza1978intersection,frankl2016invitation} from extremal set theory.

\begin{definition}($(n, k, L)$-system). 
Let $X$ be an $n$-element finite set and $L=\{l_1, l_2, \cdots, l_s\}$ be a set of non-negative integers. A family of $k$-element subsets of $X$ denoted by $\mathcal F=\{A_1, A_2, \cdots, A_{|\mathcal F|}\}$ is called an $(n, k, L)$-system if 
\begin{align}
|A_i \cap A_j| \in L,
\end{align}
for every $i \neq j$.
\end{definition}
We now recall the following upper bound on the maximum size $(n, k, L)$ systems denoted by $m(n, k, L)$.
% \begin{lemma}(Ray-Chaudhuri and Wilson Inequality \cite{ray1975t})
% \label{lemma:Ray-Chaudhuri - Wilson}
% \begin{align}
%      |\mathcal F| \leq \binom{n}{s}.
% \end{align}
% \end{lemma}
% \begin{lemma}(Deza, Erd\"{o}s and Frankl Inequality \cite{deza1978intersection}) 
% \label{lemma:Deza-Erdos-Frankl}\\
% When $n>n_0(k)$, we have
% \begin{align}
%     |\mathcal F| \leq \prod\limits_{i=1}^{s} \frac{n-l_i}{k-l_i}.
% \end{align}
% \end{lemma}

\begin{lemma}
\label{lemma:extremalsettheory}
For any $(n, k, L=\{0, 1, \cdots, s-1\})$-system, we have
\begin{align}
    m(n, k, L)\leq \frac{\binom{n}{s}}{\binom{k}{s}}.
\end{align}
\end{lemma}

We now prove Theorem \ref{thm:impossibility} based on Lemma \ref{lemma:extremalsettheory}.
\begin{proof}[Proof of Theorem \ref{thm:impossibility}]
A necessary condition for the privacy requirement to be satisfied is that any two rows $\mathbfsl b_i, \mathbfsl b_j$ of the matrix $\mathbf B$ satisfy the following 
\begin{align}
    \mathrm{supp(\mathbfsl b_i)} \cap \mathrm{supp(\mathbfsl b_j)} \leq K-\floor*{T/2}.
\end{align}
To see this, we note that if this condition is not satisfied then we have 
\begin{align}
    \| \mathbfsl b_i-\mathbfsl b_j \|_0 <T, 
\end{align}
and the privacy requirement is violated. Finally, based on Lemma \ref{lemma:extremalsettheory}, we have 
\begin{align*}
    R_{\mathrm{max}} \leq \frac{\binom{N}{K-\floor*{T/2}+1}}{\binom{K}{K-\floor*{T/2}+1}}.
\end{align*}
\end{proof}

It is also worth noting that similar bounds can be derived through Johnson's bound (See Chapter 17, Corollary 5 in \cite{macwilliams1977theory}).\\
% When $N=8, K=6$ and $T=2$, our upper bound gives $R_{\mathrm{max}}\leq 28$. However, our construction in this case has $R=4$. This gap between our construction and our bound follows since the condition in Equation (\ref{eqn:necessary}) is a necessary condition, but not sufficient. To see this, consider the following example.
% \begin{example}
% Consider the following codebook with  $N=6$ and $K=4$
% \begin{equation}
% \mathbf B=
% \begin{bmatrix}[cccccc]
% 1 & 1 & 1 & 1 & 0 & 0\\
% 0 & 0 & 1 & 1 & 1 & 1 \\
% 1 & 1 & 0 & 0 & 1 & 1  
% \end{bmatrix}.
% \end{equation}
% In this example, the user sets satisfy the condition in Equation (\ref{eqn:necessary}) for $T=4$. However, this codebook does not ensure a privacy of $T=4$ as 
% \begin{equation}
%     [1,-1,1] \ \mathbf B=[2,2,0,0,0,0].
% \end{equation}
% \end{example}



% Next, we provide the proof of Theorem \ref{thm:secondbound}.
% \begin{proof}
% We use the inclusion-exclusion principle and obtain:
% \begin{align*}
%   N & \geq  |\cup_{i = 1}^m S_i| \\
%   & \geq \sum_{i=1}^m |S_i| - \sum_{i\neq j} |S_i\cap S_j| \\
%   & \geq mK - {m \choose 2} t \\
%   & \geq mK - \frac{t m^2}{2}. 
% \end{align*}

% The function $mK - t m^2/2$ as a function of $m\geq 0$ is quadratic and attains its maximum at $m = T/t$ with function value $\frac{K^2}{2t}$. Hence, if $N\leq \frac{K^2}{2t}$, it implies a constraint on $m$: $m$ is upper bounded by the smaller root of the equation
% \begin{align*}
%     \frac{t m^2}{2} - mK + N = 0. 
% \end{align*}
% The smaller root of the equation above is given by
% \begin{align*}
%     m_* & = \frac{K - \sqrt{K^2 - 2tN}}{t} \\
%     & = \frac{K^2 - (K^2 - 2tN)}{t (K + \sqrt{K^2 - 2tN})} \\
%     & = \frac{2N}{K + \sqrt{K^2 - 2tN}} \\
%     & \leq \frac{2N}{K}. 
% \end{align*}
% \end{proof}

==> App_New_Convergence.tex <==
In this appendix, we  discuss extending the convergence proof of \cite{karimireddy2020scaffold} to our setting. Since we closely follow \cite{karimireddy2020scaffold}, we mainly here focus on the differences. The main difference between the two settings is that the number of participating users in \cite{karimireddy2020scaffold} is fixed as $|\mathcal S^{(t)}|=K$ across all rounds as \emph{dropouts} are not considered, whereas it may change in our case between the rounds based on the availability of the users. Specifically, the server in our case aims to choose $K$ users at each round. If this is not possible due to the dropouts, the server skips this round. That is,  $|\mathcal S^{(t)}| \in \{0, K\}$ and $\mathbb E[|\mathcal S^{(t)}|]=C$, where we recall that $C$ is the average aggregation cardinality that depends on the desired multi-round privacy guarantee $T$.


Next, we recall the setting and the assumptions of \cite{karimireddy2020scaffold}. In \cite{karimireddy2020scaffold}, the problem is formalized as minimizing a global loss function as follows
\begin{equation}
    \min_{\mathbfsl{x}} L(\mathbfsl{x}) \text{ s.t.  } 
    L(\mathbfsl{x}) = \frac{1}{N} \sum_{i=1}^N  L_i (\mathbfsl{x}),
\end{equation} 
where $L$ is bounded from below by $L^*$, the loss function of user $i$ $L_i$ is $\rho$-smooth and  $g_i(\mathbfsl x)=\nabla L_i(\mathbfsl x, \zeta_i)$ is an unbiased stochastic gradient of $L_i$ with variance bounded by $\sigma^2$. Furthermore, following the assumptions of \cite{karimireddy2020scaffold}, we consider the following assumptions.   \\
\textbf{Assumption 1}. $(G, B)$-Bounded Gradient Dissimilarity (BGD). There exists constants $G \geq 0$ and $B \geq 1$ such that  
\begin{align}
    \frac{1}{N} \sum_{i=1}^{N} \lVert \nabla L_i(\mathbfsl x)\rVert^2 \leq G^2+B^2 \lVert \nabla L_i(\mathbfsl x)\rVert^2, \forall \mathbfsl x,
\end{align}
and when $\{L_i\}$ are convex, this assumption can be relaxed as 
\begin{align}
    \frac{1}{N} \sum_{i=1}^{N} \lVert \nabla L_i(\mathbfsl x)\rVert^2 \leq G^2+2 \rho B^2 (L(\mathbfsl x)-L^*) , \forall \mathbfsl x.
\end{align}
\textbf{Assumption 2}. $\delta$-Bounded Hessian Dissimilarity (BHD).
\begin{align}
    \lVert \nabla^2 L_i(\mathbfsl x)-\nabla^2 L(\mathbfsl x)\rVert \leq \delta, \forall \mathbfsl x,
\end{align}
and $L_i$ is $\delta$-weakly.\\
\textbf{Assumption 3}. $L_i$is $\mu$-convex for $\mu \geq 0$ and satisfies
\begin{align}
    \langle \nabla L_i(\mathbfsl x), \mathbfsl y - \mathbfsl x \rangle \leq - \left( L_i(\mathbfsl x)- L_i(\mathbfsl y)+ \frac{\mu}{2} \lVert \mathbfsl x-\mathbfsl y\rVert^2 \right),  \text{for any} \ i, \mathbfsl x, \mathbfsl y,
\end{align}
where $\mu$ can be $0$ (general convex case).\\
\textbf{Assumption 4}. $g_i(\mathbfsl x)= \nabla L_i(\mathbfsl x; \zeta_i)$ is an unbiased stochastic gradient of $L_i$ with bounded variance. That is, we have
\begin{align}
    \mathbb E \left[\lVert g_i(\mathbfsl x)-\nabla L_i(\mathbfsl x) \rVert \right] \leq \sigma^2, \text{for any} \ i, \mathbfsl x.
\end{align}
\textbf{Assumption 5}. $\{L_i\}$ are $\rho$-smooth and satisfy 
\begin{align}
    \lVert \nabla L_i(\mathbfsl x)-\nabla L_i(\mathbfsl x) \rVert \leq \rho \lVert \mathbfsl x - \mathbfsl y \rVert, \text{for any} \ i, \mathbfsl x, \mathbfsl y. 
\end{align}
It is also worth noting that when $\{L_i\}$ are convex and $\mathbfsl x^*$ this assumption implies that 
\begin{align}
    \frac{1}{2 \rho N} \sum_{i=1}^{N} \lVert \nabla L_i(\mathbfsl x)-L_i(\mathbfsl x^*)\rVert \leq L(\mathbfsl x)-L^*,
\end{align}
and when $L_i$ is twice differentiable this assumption implies that $\lVert \nabla^2 L_i(\mathbfsl x)\rVert \leq \rho$ for any $\mathbfsl x$. 


We now recall the global and the local updates of the setting considered in \cite{karimireddy2020scaffold}. $\mathbfsl x^{(t)}$ is the global model after round $t$ and $\mathbfsl x_{i,e}^{(t)}$ is the local model of user $i$ in round $t$ and local step $e$. In round $t$, the server selects a subset of users $\mathcal S^{(t)}$.  Each user then copies the global model $\mathbfsl x_{i, 0}^{(t)}=\mathbfsl x^{(t-1)}$ and performs $E$ local update steps as follows
\begin{align}
    \mathbfsl x_{i, e}^{(t)} \coloneqq \mathbfsl x_{i, e-1}^{(t)}-\eta_l g_i(\mathbfsl x_{i, e-1}^{(t)}), 
\end{align}
where $\eta_l$ is the local step size. The users then send their updates and the server  updates the global model as follows 
\begin{align}
    \mathbfsl x^{(t)} \coloneqq \mathbfsl x^{(t-1)}+\frac{\eta_g}{K} \sum_{i \in \mathcal S} (\mathbfsl x_{i, E}^{(t)} -\mathbfsl x^{(t-1)}),
\end{align}
where $\eta_g$ is the global step size. Finally, the output is given by 
\begin{align}
    \overline{\mathbfsl x}^{(J)}=\overline{\mathbfsl x}^{(t-1)} \ \text{with probability} \ \frac{\theta_t}{\sum_\tau \theta_\tau} \text{for} \ t \in \{1, \cdots, J+1\}
\end{align}
for some weights $\{\theta_t\}$, where $J$ is the total number of rounds.
Next, we restate the convergence Theorem of \cite{karimireddy2020scaffold}.  

\begin{theorem*}
 Suppose that $\{L_i\}$ satisfy Assumptions $1, 4$ and $5$. Then for each of the following cases there exists weights $\{\theta_t\}$ and local step sizes $\eta_l$ such that for any global step size $\eta_g \geq 1$, we have
\begin{itemize}
    \item \textbf{Strongly convex.} If $\{L_i\}$ satisfy Assumption $3$ for $\mu>0$, $\eta_l \leq \frac{1}{8(1+B^2)\rho E \eta_g}$, $J \geq \frac{8(1+B^2) \rho}{\mu}$, then 
    \begin{align}
        \mathbb E \left[ L(\overline{\mathbfsl x}^J)\right]-L(\mathbfsl x^*) \leq \tilde{ \mathcal O} \left( \frac{M^2}{\mu J E K}+\frac{\rho G^2}{\mu^2 J^2}+\mu D^2 \exp{ \left(-\frac{\mu}{16(1+B^2) \rho}J \right)} \right).
    \end{align}
    \item \textbf{General convex.} If $\{L_i\}$ satisfy Assumption $3$ for $\mu=0$, $\eta_l \leq \frac{1}{8(1+B^2)\rho E \eta_g}$, $J \geq 1$, then
      \begin{align}
        \mathbb E \left[ L(\overline{\mathbfsl x}^J)\right]-L(\mathbfsl x^*) \leq \mathcal O \left( \frac{MD}{\sqrt{J E K}}+\frac{D^{4/3} (\rho G^2)^{1/3}}{(J+1)^{2/3}}+\frac{B^2 \rho D^2}{J} \right).
    \end{align}
    \item \textbf{Non-convex.} If $\{L_i\}$ satisfy Assumption $1$ and $\eta_l \leq \frac{1}{8(1+B^2)\rho E \eta_g}$, then 
       \begin{align}
        \mathbb E \left[ \lVert \nabla L (\overline{\mathbfsl x}^J) \rVert^2\right] \leq \mathcal O \left( \frac{\rho M \sqrt{F}}{\sqrt{J E K}}+\frac{F^{2/3} (\rho G^2)^{1/3}}{(J+1)^{2/3}}+\frac{B^2 \rho F}{J} \right).
    \end{align}
\end{itemize}
where $M^2=\sigma^2(1+K/\eta_{g}^2)+E(1-K/N)G^2, D=\lVert \mathbfsl x^{0} - \mathbfsl x^* \rVert$ and $F=L(\mathbfsl x^{0})-L^*$.
\end{theorem*}
As we discussed, the main difference between our setting and the setting of \cite{karimireddy2020scaffold} is that the number of selected users in our case in each round is a  random variable  $|\mathcal S^{(t)}| \in \{0, K\}$ with mean equal to the average aggregation cardinality $C$. We now show the effect of this difference on the key lemma of \cite{karimireddy2020scaffold}. We first recall this key lemma from \cite{karimireddy2020scaffold} and then derive a simple corollary that extends this lemma to our setting.   

\begin{lemma*} (Separating Mean and Variance)[Lemma 4 in \cite{karimireddy2020scaffold}]. Let $\{\mathbfsl E_1, \mathbfsl E_2, \cdots, \mathbfsl E_w \}$ be random vectors in $\mathbb R^d$, which may not be independent. We consider the following two cases.
\begin{itemize}
    \item When $\mathbb E[\mathbfsl E_i]= \boldsymbol{\zeta}_i$ and $\mathbb E[\lVert \mathbfsl E_i-\boldsymbol \zeta_i \rVert^2] \leq \sigma^2$, then we have
    \begin{align}
    \mathbb E[\lVert \sum_{i=1}^{w} \mathbfsl E_i\rVert^2] \leq \lVert \sum_{i=1}^{w} \boldsymbol \zeta_i\rVert^2+ w^2 \sigma^2.
    \end{align}
    \item  When $\mathbb E[\mathbfsl E_i| \mathbfsl E_{i-1}, \cdots, \mathbfsl E_1]= \boldsymbol{\zeta}_i$ and $\mathbb E[\lVert \mathbfsl E_i-\boldsymbol \zeta_i \rVert^2] \leq \sigma^2$, then we have
    \begin{align}
    \mathbb E[\lVert \sum_{i=1}^{w} \mathbfsl E_i\rVert^2] \leq 2 \lVert \sum_{i=1}^{w} \boldsymbol \zeta_i\rVert^2+ 2w \sigma^2.
    \end{align}
\end{itemize}
\end{lemma*}
In this key lemma, $w$ is constant as the setting \cite{karimireddy2020scaffold} assumes the number of participating users is fixed as $K$ in every round. That is, this lemma is applied with $w=K$. In our case, however, the number of participating users is a  random variable. Hence, we consider this case in the following corollary. 
\begin{corollary} Let $\{\mathbfsl E_1, \mathbfsl E_2, \cdots, \mathbfsl E_{W} \}$ be random vectors in $\mathbb R^d$, which may not be independent and $W \in \{0, w\}$ is a  random variable that is independent of $E_i$ and $\mathbb E[W]=\mu_W$. We consider the following two cases.
\begin{itemize}
    \item When $\mathbb E[\mathbfsl E_i]= \boldsymbol{\zeta}_i$ and $\mathbb E[\lVert \mathbfsl E_i-\boldsymbol \zeta_i \rVert^2] \leq \sigma^2$, then we have
    \begin{align}
    \mathbb E[\lVert \sum_{i=1}^{W} \mathbfsl E_i\rVert^2] \leq \frac{\mu_W}{w} \lVert \sum_{i=1}^{w} \boldsymbol \zeta_i\rVert^2+ w \mu_W \sigma^2.
    \end{align}
    \item  When $\mathbb E[\mathbfsl E_i| \mathbfsl E_{i-1}, \cdots, \mathbfsl E_1]= \boldsymbol{\zeta}_i$ and $\mathbb E[\lVert \mathbfsl E_i-\boldsymbol \zeta_i \rVert^2] \leq \sigma^2$, then we have
    \begin{align}
    \mathbb E[\lVert \sum_{i=1}^{W} \mathbfsl E_i\rVert^2] \leq 2 \frac{\mu_W}{w}\lVert \sum_{i=1}^{w} \boldsymbol \zeta_i\rVert^2+ 2\mu_W \sigma^2.
    \end{align}
\end{itemize}
\end{corollary}
This is the main difference between our setting and the setting considered in \cite{karimireddy2020scaffold} and the rest of the proof follows similarly. Similar to Theorem \ref{thm:convergence}, we can see that the average aggregation cardinality $C$ controls the convergence rate and hence there is a trade-off between the multi-round privacy $T$ and the convergence rate. 


==> old_App_Random_Selection.tex <==
In this appendix, we first theoretically study the multi-round privacy  of two random user selection strategies, and show that they have a very weak multi-round privacy of $T=1$ with high probability (for the case where $p_i=p, \forall i \in [N]$).  Furthermore, we also provide additional experiments showing that the server can reconstruct the local models of all users with high accuracy when a random selection strategy is used. In the theoretical analysis, to simplify the problem, we assume that the model of the users have converged and don't change from one round to the next. However, in the experiments, we empirically evaluate the error in approximating the individual models of the users (via least-squares error estimation), and show that the server can approximate individual models with very small error.
% Finally, we also show empirically that the local models cannot be reconstructed when \namespace is used. 

\subsection{Theoretical Analysis of the Random Selection Strategies}
We start by our theoretical results, where we consider the following two random selection schemes.
\begin{enumerate}[leftmargin=0.6cm]
    \item \textbf{$K$-uniform Random Selection}. In this scheme, at round $t$, $K$ users are selected uniformly at random from the set of available users $\mathcal U^{(t)}$ if $|\mathcal U^{(t)}| \geq K$. Otherwise, the server skips this round. 
    \item \textbf{I.I.D Random Selection}. In this scheme, at round $t$, each  user is selected with probability $ \frac{K}{N(1-p)}$ independently from the other available users, where $K < N(1-p)$. Hence, the expected number of selected users at each round is $K$ user.
\end{enumerate}
For both schemes, we show that the server can reconstruct all individual models after $N$ rounds in the worst-case scenario (assuming that the models do not change over $N$ rounds). Specifically, we show that the participation matrices in both schemes have full rank with high probability after $N$ rounds. This, in turn, implies that the server can reconstruct all local models after $N$ rounds with high probability in both schemes.  We provide our results formally next in Theorem \ref{thm:random-selection-multi-round}.

\begin{theorem}\label{thm:random-selection-multi-round} (Random Selection Schemes have multi-round privacy guarantee of $T=1$).
\begin{enumerate}[leftmargin=0.6cm]
    \item Consider the $K$-uniform random selection scheme, where $\min(K,N-K) \geq cN$. In this scheme, the server can reconstruct all individual models of the $N$ users after $N$ rounds with probability at least
    \begin{align}
        1-2e^{-c'N},
    \end{align}
    for some constant $c'>0$ that depends on $c$.
    
    \item Consider the i.i.d random selection scheme, where the users are selected according to Bern($\frac{K}{N(1-p)}$) distribution and let $t=K/N$. In this scheme, the server can reconstruct the individual models of the $N$ users after $N$ rounds with probability at least 
    \begin{align}
    1 - 2N(1-t)^N - (1+o_N(1)) N(N-1)(t^2 + (1-t)^2)^N,
    \end{align}
    which converges to $1$ exponentially fast if $t \in (0, 1/2)$ is a fixed constant. 
%     In particular, if $t = 1/2$, then this probability is at least 
%     \begin{align}
%     1- (1/2 + o_N(1))^N.
%     \end{align}
\end{enumerate}
\end{theorem}

\begin{proof}
We first note that if the participation matrix has full rank after $N$ rounds, then the server  can reconstruct the model of each individual user. Hence, we analyze the probability of the $N \times N$ participation matrix being full rank. We now consider each scheme separately. 
\begin{enumerate}[leftmargin=0.6cm]
    \item In the $K$-uniform random selection scheme, the probability that the participation matrix after $N$ rounds $\mathbf P^{(N)}$ has full rank is lower-bounded as follows (T. Tran, 
2020), when $\min(K,N-K) \geq cN$, 
\begin{align*}
    \Pr[\mathbf P^{(N)} \ \text{has full rank}] \geq 1-2e^{-c'N},
\end{align*}
for some constant $c'>0$ that depends on $c$. Hence, it follows that the server can reconstruct all individual models with probability at least $1-2e^{-c'N}$.

\item In the i.i.d random selection scheme, the probability that the participation matrix after $N$ rounds $\mathbf P^{(N)}$ has full rank is lower-bounded as follows (V. Jain et al., 2020)
\begin{align*}
 \Pr[\mathbf P^{(N)} \ \text{has full rank}] \geq  1 - 2N(1-t)^N - (1+o_N(1)) N(N-1)(t^2 + (1-t)^2)^N,
\end{align*}
which converges to $1$ exponentially fast if $t=K/N \in (0, 1/2)$ is a fixed constant. Hence, it follows that the probability the server can reconstruct all individual models is lower-bounded by the same probability.  
% Moreover, when $p=1/2$, we have \cite{tikhomirov2020singularity}
% \begin{align*}
%     \Pr[\mathbf P^{(N)} \ \text{is full rank}] \geq 1- (1/2 + o_N(1))^N.
% \end{align*}
\end{enumerate}
\end{proof}

\begin{remark}\normalfont 
Our experimental results in Section \ref{sec:Experiments} also show that the multi-round privacy guarantee of the $K$-uniform random selection scheme goes to $1$ after almost $N$ rounds as shown in Fig. \ref{fig:priavcy}.
\end{remark}

\subsection{Experimental Results}
We now empirically evaluate the error in approximating the individual models of the users (via least-squares error estimation), and show that the server can approximate individual models of all users with very small error. To do so, we implement a reconstruction algorithm utilizing the least-squares method, and measure the $L_2$ distance between the original model and reconstructed model.
% We further aim to reconstruct the local models in \namespace scheme with various target multi-round privacy guarantees $T$ to figure out how the multi-round privacy guarantee affects the reconstruction performance by measuring the $L_2$ distance between the original models and reconstructed models.
% To do so, we measure the $l_2$ distance between the original model and reconstructed model.

We consider a FL setting with $N=40$ users, where the server aims to choose $K=8$ users at every round, to train the CNN in \cite{mcmahan2016communication} on the MNIST dataset with IID setting. After a sufficiently large number of rounds $t_0$, the global model at the server converges and does not change much across the rounds, which results in that local models also do not change much across the rounds. Then, we have
\begin{equation}
    \mathbf{X}^{(t_0;t_1)}_{\text{global}} = \mathbf{P}^{(t_0;t_1)}
    \mathbf{X}^{(t_0)}_{\text{individual}} + \mathbf{Z},
    % \mathbf{X}^{(t_0;t_1)}_{\text{global}} = \mathbf{P}^{(t_0;t_1)} \mathbf{X}^{(t_0)}_{\text{individual_avg}} + \mathbf{Z},
\end{equation}
where $\mathbf{X}^{(t_0;t_1)}_{\text{global}}$ denotes the concatenate of the global models from round $t_0$ to round $t_1 - 1$, i.e., $\mathbf{X}^{(t_0;t_1)}_{\text{global}} = \left[ \mathbfsl{x}^{(t_0)}, \ldots \mathbfsl{x}^{(t_1-1)} \right]^{\top}\in \mathbb{R}^{(t_1-t_0)\times d}$ for $t_1 > t_0$,
$\mathbf{P}^{(t_0;t_1)} \in \{0,1\}^{(t_1-t_0)\times N}$ is the participation matrix from round $t_0$ to round $t_1-1$,
$\mathbf{X}^{(t_0)}_{\text{individual}}$ denotes the concatenate of the individual models at round $t_0$, i.e., $\mathbf{X}^{(t_0)}_{\text{individual}} = \left[ \mathbfsl{x}^{(t_0)}_1, \ldots, \mathbfsl{x}^{(t_0)}_N \right]^{\top}\in \mathbb{R}^{N\times d}$, and $\mathbf{Z}$ denotes the perturbation (or noise) incurred by the local updates across the rounds. 

% When the $\mathbf{P}^{(t_0;t_1)}$ is full rank($=N$), 
The server can then estimate $\mathbf{X}^{(t_0)}_{\text{individual}}$ by utilizing the least-squares method as follows
\begin{equation}\label{eq:recon_ind}
    \hat{\mathbf{X}}^{(t_0)}_{\text{individual}} = \left( {\mathbf{P}^{(t_0;t_1)}}^\top \mathbf{P}^{(t_0;t_1)} \right)^{-1} {\mathbf{P}^{(t_0;t_1)}}^\top \mathbf{X}^{(t_0;t_1)}_{\text{global}},
\end{equation}
% On the other hand, when \namespace is used, the server cannot reconstruct the individual model from \eqref{eq:recon_ind} because $\mathbf{P}^{(t_0;t_1)}$ cannot be full rank. 
% This is due to the fact that at each round, users in the same batch either participate together or not participate at all. 
% The best that the server can reconstruct is partial aggregate of the local models of users in the same batch of size $T$.
and we measure the reconstruction error as follows 
\begin{equation}\label{eq:recon_error}
   e^{(t_0)}_i = \frac{\lVert \mathbfsl{x}_i^{(t_0)} - \hat{\mathbfsl{x}}_i^{(t_0)} \rVert^2}{\lVert \mathbfsl{x}_i^{(t_0)} \rVert^2},
    % e^{(t_0)} = \frac{1}{N}\sum_{i=1}^{N}e^{(t_0)}_i = \frac{1}{N}\sum_{i=1}^{N}\frac{\lVert \mathbfsl{x}_i^{(t_0)} - \hat{\mathbfsl{x}}_i^{(t_0)} \rVert^2}{\lVert \mathbfsl{x}_i^{(t_0)} \rVert^2}, 
\end{equation}
% $e^{(t_0)} = \frac{1}{N}\sum_{i=1}^{N}e^{(t_0)}_i = \frac{1}{N}\sum_{i=1}^{N}\frac{\lVert \mathbfsl{x}_i^{(t_0)} - \hat{\mathbfsl{x}}_i^{(t_0)} \rVert^2}{\lVert \mathbfsl{x}_i^{(t_0)} \rVert^2}$ 
where $\hat{\mathbfsl{x}}_i^{(t_0)}$ denotes the reconstructed model of user $i$, which corresponds to $i$-th row of $\hat{\mathbf{X}}^{(t_0)}_{\text{individual}}$ in \eqref{eq:recon_ind}.
Figure \ref{fig:histo_error} shows the histogram of the reconstruction error of the individual models of $N=40$ users with $t_0=260$ and $t_1=300$.
We observe that the $K$-uniform random selection scheme has a very small average reconstruction error $\frac{1}{N}\sum_{i=1}^{N}e^{(t_0)}_i=1.72\times10^{-3}$, which implies that the server can reconstruct all local models as the $K$-uniform random selection scheme has the multi-round privacy guarantee $T=1$.

\begin{figure}[htb!]
    \centering
    \includegraphics[scale=0.55]{figures/error_histo.eps}
  \caption{\footnotesize Histogram of the reconstruction error defined in \eqref{eq:recon_error} of $N=40$ users when the $K(=8)$-uniform random selection scheme is used to train the CNN \cite{mcmahan2016communication} on the MNIST dataset.}
    \label{fig:histo_error}
\end{figure}

% Table \ref{tbl:l2dist_construction} shows the reconstruction error in \eqref{eq:recon_error} of three scheme, $K$-uniform random selection, \namespace($T=2$), and \namespace($T=4$) with $t_0= 350$ and $t_1 = 400$. We use the same hyperparameters provided in Appendix \ref{app:hyperparameters}.
% We can observe that $K$-uniform random selection has much smaller value of error than other two schemes, which implies that the server can reconstruct all local models as $K$-uniform random selection ensures the multi-round privacy guarantee of $T=1$.

% \begin{table}[h!]
% \small
% \caption{Reconstruction error defined in \eqref{eq:recon_error} with $N=40$, $K=8$, $t_0= 350$, and $t_1 = 400$.}
% % \caption{Average value of $L_2$ distance between the original models and reconstructed models.}
% \label{tbl:l2dist_construction}
% % \vskip 0.15in
% \begin{center}
% % \begin{small}
% % \begin{sc}
% \begin{tabular}{ccc}
% \toprule
% $K$-uniform random selection ($T=1$) & \namespace($T=2$)  & \namespace($T=4$)\\
% \midrule
% $0$  &  $0$ &  $0$ \\
% % Weighted random selection &  $65.06\%$ &  $47.89\%$ \\
% \bottomrule
% \end{tabular}
% % \end{sc}
% % \end{small}
% \end{center}
% \end{table}


\begin{thebibliography}{1}
	\bibitem[T. Tran,2020]{Tran200}
		T. Tran,
		``The smallest singular value of random combinatorial matrices'', arXiv preprint arXiv:2007.06318 (2020).
	\bibitem[V. Jain et al.,2020]{Jain2020}
		V. Jain, A. Sah, and M. Sawhney,
		``Singularity of discrete random matrices II'', arXiv preprint arXiv:2010.06554 (2020).
\end{thebibliography}
